Locally Uniform Hashing

Hashing is a common technique used in data processing, with a strong impact on the time and resources spent on computation. Hashing also affects the applicability of theoretical results that often assume access to (unrealistic) uniform/fully-random hash functions. In this paper, we are concerned with designing hash functions that are practical and come with strong theoretical guarantees on their performance. To this end, we present tornado tabulation hashing, which is simple, fast, and exhibits a certain full, local randomness property that provably makes diverse algorithms perform almost as if (abstract) fully-random hashing was used. For example, this includes classic linear probing, the widely used HyperLogLog algorithm of Flajolet, Fusy, Gandouet, Meunier [AOFA 97] for counting distinct elements, and the one-permutation hashing of Li, Owen, and Zhang [NIPS 12] for large-scale machine learning. We also provide a very efficient solution for the classical problem of obtaining fully-random hashing on a fixed (but unknown to the hash function) set of $n$ keys using $O(n)$ space. As a consequence, we get more efficient implementations of the splitting trick of Dietzfelbinger and Rink [ICALP'09] and the succinct space uniform hashing of Pagh and Pagh [SICOMP'08]. Tornado tabulation hashing is based on a simple method to systematically break dependencies in tabulation-based hashing techniques.

==> app.tex <==
\section{Code}\label{app:code}
The following is a simple implementation of tornado tabulation for 32-bit keys, with \(\Sigma = [2^{8}]\), \(c=4\), \(d=3\), and \(\cR=2^{32}\).
Besides the key \texttt{x} the function takes as input an array of \(c+d\) tables of size \(\ssigma\), each an independently drawn 64-bit value.
The 64-bit entries allow us to perform all lookups for each character \(x_i\) or \(\derive x_i\) just once, and xor it onto the preliminary result \texttt{h} which also contains the derived characters and the twisted \(\derive x_c\).
Note that the key is read in reverse, such that \(x_1\) corresponds to the least significant bits and \(x_c\) is \texttt{x >>= 24}.

The first loop takes care of lookups related to the (unaltered) characters \(x_1, \dots, x_{c-1}\) while the lookups based on \(\derive x_c, \dots, \derive x_{c+d}\) are handled in the second loop.
For each iteration the 8 remaining least significant bits are cast to a byte which is used for indexing into the appropriate table \texttt{H[i]}.

\begin{lstlisting}[language=C,basicstyle=\footnotesize]
	INT32 Tornado(INT32 x, INT64[7][256] H) {
		INT32 i;
		INT64 h=0;
		INT8 c;
		for (i=0;i<3;i++) {
			c=x;
			x>>=8;
			h^=H[i][c];
		}
		h^=x;
		for (i=3;i<7;i++) {
			c=h;
			h>>=8;
			h^=H[i][c];
		} 
		return ((INT32) h); 
	}
\end{lstlisting}

Now the tornado-mix from 64 to 64
bits plus 64 bits for derivation, using 8-bit characters except the last two which are 16 bits,
so in the end 11 8-bit tables
and 2 16-bit tables.

\begin{lstlisting}[language=C,basicstyle=\footnotesize]
    INT64 Tornado(INT64 x, INT128[11][256] H8, INT64[2][65536] H16) {
        INT32 i;
        INT128 h=0;
        INT8 a;
        INT16 b1,b2;
        for (i=0;i<7;i++) {
        	a=x;
        	x>>=8;
        	h^=H8[i][a];
        }
        h^=x;
        for (i=7;i<11;i++) {
        	a=h;
        	h>>=8;
        	h^=H8[i][a];
        } 
        b1=h; h>>=16;
        b2=h; h>>=16;
        h^=H16[i][b1]^H16[i][b2];
        return ((INT64) h); 
    }
\end{lstlisting}


==> intro-linear-probing.tex <==
\section{Linear Probing with Tornado Tabulation}\label{sec:linear-probing}



In this section we show how to formally apply our framework to obtain results on linear probing with tornado tabulation.
We present the following main result comparing the performance of linear probing with tornado tabulation to that of linear probing using fully random hashing on a slightly larger keyset.

\begin{theorem}\label{thm:linearprobing}
  Let \(S, S^* \subseteq \Sigma^c\) be sets of keys of size \(n\) and \(n^* = (1+15\sqrt{\log(1/\delta)/\ssigma})n\), respectively, for some \(\delta \in (0,1/6)\).
  Let $T$, $T^*$ be arrays of size \(m\), a power of two. Now consider inserting the keys in \(S\) (\(S^*\)) into $T$ ($T^*$)  with linear probing using tornado tabulation (fully random hashing).
Let $X$ and $X^*$ be the number of comparisons performed when inserting a new key \(x\) in each of \(T\) and \(T^*\) (i.e., $x\notin S\cup S^*$).
Given the restrictions listed below there exists an event $\calE$ with \(\Pr(\calE) \geq 1 - \ld(1/\ssigma + 6\delta + 61 \log n \cdot  \DepProb(\ssigma/2, d, \Sigma)\rd)\) such that, conditioned on $\calE$, \(X\) is stochastically dominated by \(X^*\). \\
Restrictions:
\begin{itemize}
\item \(n/m \leq 4/5\)
\item \(\ssigma \geq 2^{16}\)
\item \(\ssigma \geq 30 \cdot \log n\)
\item \(\sqrt{\log (1/\delta)/\ssigma} \leq 1/18\) %% to keep difference between \(n\) and \(n^*\) small enough for proof in \cref{subsec:comparison-fully} to apply.
\end{itemize}
\end{theorem}

From~\Cref{thm:linearprobing}, it follows that linear probing using tornado tabulation achieves the same expected number of comparison as in the fully random setting,
a proof is given in \cref{subsec:linearprobing-expectation}.

\begin{corollary}\label{cor:linearprobing}
  Setting \(\delta = \Theta(1/\ssigma)\), \(d \geq 5\), \(\log n \leq o(\ssigma)\) in \cref{thm:linearprobing} we have
  %% With the definitions from \cref{thm:linearprobing}
  \[
  \Ep{X} \leq \Ep{X^*} + o(1)\, .
  \]
\end{corollary}

The result of \cref{cor:linearprobing} is to be contrasted with previous work on practical implementations of linear probing.
While Knuth's analysis serves as evidence of linear probing's efficieny in terms of the number of comparisons performed, 
the advantage of linear probing (over other hash table implementations) is that each sequential memory access is much faster than
the random memory access  we do  for the first probe at $T[h(x)]$. How much faster depends on the computer system as does the cost of increasing the memory to reduce the load.  
Some experimental 
studies~\cite{black98linprobe,heileman05linprobe,thorup11timerev} have
found linear probing to be the fastest hash table organization for
moderate load factors (30-70\%). If the load is higher, we could
double the table size.

However, using experimental benchmarks to decide the hash table organization is only meaningful if the experiments are representative of the key sets on which linear probing would be employed. Since fully random hashing cannot be efficiently implemented, we might resort to weaker hash functions for which there could be inputs leading to much worse performance than in the benchmarks. The sensitivity to a bad choice of the hash function
led \cite{heileman05linprobe} to advice \emph{against} linear
probing for general-purpose use.
Indeed, Mitzenmacher and Vadhan \cite{mitzenmacher08hash} have proved that 2-independent hashing
performs as well as fully random hashing if the input has enough entropy. However, \cite{thorup12kwise,patrascu10kwise-lb} have shown that with the standard  2-independent linear hashing scheme, if the input is a dense set (or more generally, a dense subset of an arithmetic sequence), then linear probing
becomes extremely unreliable and the expected probe length increases from Knuth's $\frac{1+1/\eps^2}2$ to $\Omega(\log n)$, while the best known upper bound in this case is $n^{o(1)}$~\cite{knudsen2016linear}.\footnote{We note that if we only know that the hash function is $2$-independent, then the lower bound for the expected probe length is $\Omega(\sqrt{n})$ and this is tight.~\cite{thorup12kwise,patrascu10kwise-lb}}

In a breakthrough result, Pagh, Pagh and Ru{\v z}i{\'c}~\cite{pagh07linprobe} showed that if we use 5-independent hashing and
the load gap $\eps=\Omega(1)$, then the expected probe length is 
constant. P{\v a}tra{\c s}cu  and Thorup~\cite{patrascu12charhash} generalized this to an $O(1/\eps^2)$ bound for arbitrary
$\eps$, and showed that this
also holds for simple tabulation
hashing. However, in both
cases, the analysis hides
unspecified large constants
in the $O$-notation. Thus, with
these hashing schemes,
there could still be inputs for
which linear probing performs, say,  10 times worse in expectation, and then we would be better off using chaining.

Our result is of a very different nature.
We show that whp, for any given query key $x$, the probe length 
corresponding to $h(x)$ when we use tornado tabulation hashing is stochastically dominated by the probe length in a linear probing table that hashes slightly more keys but uses fully random hashing. In particular, this implies that whp,  the expected
probe length with tornado tabulation hashing is only a factor $1+o(1)$ away from Knuth's $\frac{1+1/\eps^2}2$. We get
this result without having to revisit Knuth's analysis from \cite{knuth63linprobe}, but simply
because we know that we are almost as good as fully random hashing, in a local sense that is sufficient for bounding the probe length (see \cref{subsec:linearprobingproof}).

As a further consequence of our results, we get that any benchmarking with  random keys that we do in order to set system parameters will  be representative for all possible sets of input keys. Moreover, the fact that tornado tabulation hashing only needs locality to perform almost as well as fully random hashing means that our arguments also work for other variants of linear probing.  For instance, ones where the maintenance of the hash table prioritizes the keys depending on when they were inserted, as first suggested in 
\cite{amble1974ordered}. Examples of this include Robin hood hashing where keys
with the lowest hash value come first \cite{celis1985robin} or time-reversed linear probing \cite{thorup11timerev} where the latest arrival comes first. In all these cases, tornado tabulation hashing performs almost as well as with fully-random hashing.


\subsection{Proof of~\cref{thm:linearprobing}}\label{subsec:linearprobingproof}
%% We let \(\eps = 1 - \alpha = 1 - n/m\) denote the fraction of unoccupied cells in \(T\).
We let $\alpha = n/m$ denote the fill of the hash table and $\eps = 1-\alpha$.
The basic combinatorial measure that we study and employ is the \emph{run length}: If cells \(T[a]\), \(T[a+1], \dots, T[b-1]\) are all occupied by elements from \(S\) but both \(T[a-1]\) and \(T[b]\) are freem these \(b-a\) cells are called a run of length \(b-a\).
%% The basic combinatorial measure that we study and employ is the \emph{run length}: given an element $x$ (not necessarily in the set), we define the run length of $x$ to be occupied cells of
%% $R(x,S) = \ell$ if and only position $h(x), h(x)+1, \ldots, h(x)+\ell-1$ contain keys from $S$ but $h(x)+\ell$ is empty.
Let \(R(x, S)\) be the length of the run intersecting \(T[h(x)]\) and
note that $R(x, S) +1$ is an upper bound on the number of comparisons needed to insert some element $y$ into the table when $y$ hashes to the same location as $x$.

Let \(\Delta\) be the largest power of two such that \(3\alpha\Delta + 1 \leq \ssigma/2\).
The following lemma, proven in \cref{subsec:proof-runlength}, gives an upper bound on the probability that \(h(x)\) intersects a long run.

\begin{lemma}\label{lemma:newrunlength}
  \[ \Prp{R(x, S) \geq \Delta} \leq \frac{1}{\ssigma} + 60 \log n \cdot \DepProb(\ssigma/2, d, \Sigma) \, . \]
\end{lemma}

Let \(\calA\) be the event \(\ld(R(x, S) \geq \Delta \rd)\).
Assuming \(\calA\), there exists at least one unoccupied cell in table \(T\) between \(T[h(x) - \Delta]\) and \(T[h(x)]\) and likewise between \(T[h(x)]\) and \(T[h(x) + \Delta]\).
Hence the insertion of \(x\) only depends on the distribution of the much smaller key-set \(\set{s \in S \, \big| \, \size{h(s) - h(x)} \leq \Delta}\).

The second step of our proof bounds the probability that tornado tabulation behaves like a fully random hash function when restricted to this small set of keys.
As \cref{thm:intro-random-set} doesn't apply for arbitrary intervals we will instead cover the necessary interval with three dyadic intervals.
Recall that a dyadic interval is an interval of the form $[j2^i, (j+1)2^i)$, where $i,j$ are integers.
  In the following we will exclusively consider a number of dyadic intervals all of length \(\Delta\).
  Let $I_C$ denote the dyadic interval that contains $h(x)$, and similarly let $I_R$ and $I_L$ denote the dyadic intervals to the left and right, respectively, of $I_C$.
  We further let $X_C$ be the set of keys in $S$ that hash into the interval $I_C$, i.e., $X_C = \set{x\in S \mid h(x)\in I_C}$, and similarly, $X_R$ and $X_L$ are the pre-image of $h$ in $I_R$ and $I_L$, respectively.
  Given \(\calA\), the distribution of \(X\) is completely determined by the distribution of the keys in \(X_L \cup X_C \cup X_R\) and \(h(x)\).

  The expected size of each preimage is \(\alpha \Delta\) and our choice of \(\Delta\) thus allows us to apply \cref{thm:intro-random-set} to all three intervals at once. Let \(\calB\) be the event that the keys hashing into these intervals are distributed independently:
  
  \begin{corollary}\label{lemma:dyadic-uniform}
    With probability at least \(1 - \DepProb(\ssigma/2, d, \Sigma)\), \(\tilde h(X_R \cup X_C \cup X_L \cup \set{x})\) is linearly independent, such that $h$ hashes the keys in $X_R \cup X_C \cup X_L \cup \set{x}$ independently and uniformly in their respective intervals.
  \end{corollary}

We now define the analogous terms in the fully random setting. We let $I^{*}_C$ denote the dyadic interval in $T^{*}$ that contains $\hstar(x)$ and $I^{*}_R$ and $I^{*}_L$ the right and left neighboring dyadic intervals. Similarly, we let $X^{*}_C$, $X^{*}_R$ and $X^{*}_L$ denote their preimages under $\hstar$. The following lemma compares the two experiments in terms of the sizes of these preimages, and is proven in \cref{subsec:comparison-fully}.

\begin{lemma}\label{lemma:comparison-fully}
  Let \(\calC\) be the event \(\size{X_L} \leq \size{X^*_L} \land \size{X_C} \leq \size{X^*_C} \land \size{X_R} \leq \size{X^*_R}\), then
  \[ \Prp{\calB \land \bar\calC} \leq 6\delta \]
\end{lemma}

Let \(\calC\) be the event that each of the preimages \(X_i\) contain at most as many elements as the corresponding preimage \(X_i^*\).
Finally, define \(\calE = \calA \cap \calB \cap \calC\).
We will now present a coupling \(\tilde X\) of \(X\) which, when conditioned on \(\calE\), satisfies \(\tilde X \leq X^*\).

For every realization of $\size{X_L}$, $ \size{X_C}$ and $\size{X_R}$, we consider the following random process: starting from an emtpy table of size $m$ and using the fully random $\hstar$, insert the first $\size{X_L}$ elements from $X^{*}_L$, then the first $\size{X_R}$ elements from $X^{*}_R$ and finally, the first $\size{X_C}$ elements from $X^{*}_C$ (we do not insert any more elements after this). Note that, conditioned on $\calC$, we have that it is possible to choose such elements (i.e., $\size{X_R} \leq \size{X^{*}_R}$ etc.). Now let $\tilde{X}$ denote the number of comparisons performed when inserting $x$ into the table at this point in time.

We now have that $X$ (defined for the tornado tabulation) is identically distributed as $\tilde{X}$ (defined for a fully random hash function).
This is because event $\calA$ implies that the distribution of $X$ only depends on $X_R$, $X_C$ and $X_L$.
Event $\calB$ further implies that, on these intervals, $h$ behaves like a fully random hash function.
Now note that $\tilde{X} \leq X^{*}$, since we can continue the random process and add the remaining keys in $S^{*}$ and this can only increase the number of comparisons required to insert $x$ (i.e., ``more is worse'').

Left is to compute the total probability that any of our required events fail:
\begin{align*}
  \Prp{\bar \calE} &= \Prp{\bar \calA \lor \bar \calB \lor \bar \calC} \\
  &= \Prp{(\bar \calA \lor \bar \calC) \land \calB} + \Prp{\bar \calB} \\
  &\leq \Prp{\bar \calA} + \Prp{\calB \land \bar \calC} + \Prp{\bar \calB} \\
  &\leq 1/\ssigma + 6\delta + 61 \cdot \log n \cdot \DepProb(\ssigma/2, d, \Sigma) \, .
\end{align*}
This concludes the proof.

\subsection{Proof of~\cref{lemma:comparison-fully}}\label{subsec:comparison-fully}
As \(\Delta\) is chosen to be the largest power of two such that \(3 \alpha \Delta \leq \ssigma/2\) we get \(\frac{\ssigma}{12 \alpha} \leq \Delta\).
Let \(t\) be a constant, to be decided later.
For each \(i \in \set{L, C, R}\) let \(\calE_i\) be the event (\(\size{X_i} \leq t\)) and \(\calE_i^*\) be the event (\(t \leq \size{X_i^*}\)).
\begin{align*}
  \Prp{\calB \land \bar \calC} &=
  \Prp{\calB \land \exists i \in \set{L, C, R} : \size{X_i} > \size{X_i^*}} \\
  &\leq \Prp{\calB \land \exists i \in \set{L, C, R} : \bar \calE_i \lor \bar \calE_i^*} \\
  &\leq \sum_{i \in \set{L, C, R}} \ld( \Prp{\calB \land \size{X_i} > t} + \Prp{\calB \land \size{X_i^*} < t} \rd) \\
  &\leq \sum_{i \in \set{L, C, R}} \ld( \Prp{\calB \land \size{X_i} > t} + \Prp{\size{X_i^*} < t} \rd) \\
\end{align*}

Let \(\mu = \Ep{\size{X_i}} = \Delta\alpha\),
\(k = \sqrt{3\log (1/\delta)/\mu}\) and \(t = (1+k) \mu\).
Applying the tail-bound of \cref{lemma:upper-chernoff} we have
\begin{align*}
  \Prp{\calB \land \size{X_i} > t} &= \Prp{\calB \land \size{X_i} > (1+k)\mu} \\
  &\leq \exp\ld(- k^2 \mu / 3\rd) \\
  &= \delta \, .
\end{align*}

As \(\mu = \alpha \Delta \geq \ssigma/12\) we have
\begin{align*}
  k &= \sqrt{3\log (1/\delta)/(\alpha \Delta)} \\
  &\leq \sqrt{36 \log (1/\delta) / \ssigma} \\
  &\leq 1/3 \, .
\end{align*}
As \(n^* = (1+15\sqrt{\log (1/\delta)/\ssigma})n \geq (1 + 2.5 k)n\), \(\mu^* = \Ep{\size{X_i^*}} \geq (1 + 2.5k) \mu\).
Next, let \(k^* = k \cdot \sqrt{2/3}\). Then
\begin{align*}
  \mu^* \cdot (1 - k^*) &\geq (1 + 2.5k) \cdot \mu \cdot (1 - k^*) \\
  &= (1 + 2.5k) \cdot \mu \cdot (1 - \sqrt{2/3} \cdot k) \\
  &\geq \mu \cdot (1 + k) \\
  &= t \, .
\end{align*}
Hence
\begin{align*}
  \Prp{\size{X_i^*} < t} &\leq \Prp{\size{X_i^*} < (1-k^*) \mu^*} \\
  &\leq \exp(- (k^*)^2 \mu^* / 2) \\
  &= \exp(- k^2 \mu^* / 3) \\
  &\leq \exp(- k^2 \mu / 3) \\
  &= \delta \, .
\end{align*}

Summing over the six cases we see \(  \Prp{\calB \land \exists i \in \set{L, C, R} : \size{X_i} > \size{X_i^*}} \leq 6\delta\).

\begin{comment}

Notes: \(\Prp{\size{X_i^*} < t}\) is found using standard Chernoff while \(\Prp{\size{X_i > t}}\) will rely on Chernoff-like concentration for tornado tab (if available?) or Theorem 4(1) of Fast Hashing \cite{aamand2020fast}, in some simplified form, perhaps.
Larger values \(\Delta\) brings better concentration without any side-effect (as far as I can tell, maybe our main-theorem will be sensitive to the size?), so I guess we just max out.

These Chernoff-like bounds may introduce additive factors (at least our main theorem will), so this could introduce further restrictions on the relationship between \(\eps, \ssigma\), and \(c\).

In fact, we need these Chernoff-like bounds to be query-invariant, as intervals are chosen based on \(h(x)\). Make note of this somewhere.
\end{comment}

\subsection{Proof of \cref{lemma:newrunlength}}\label{subsec:proof-runlength}
%% \cref{lemma:runlength} is awkward as it introduces asymptotics and is limited by the less impressive properties of simple tabulation.
%% The following is a sketch for how \(R(x, S)\) can be bounded purely by relying on the concentration bounds we've obtained for tornado tabulation, \cref{lemma:upper-chernoff} and \cref{lemma:large-upper-chernoff}.

Our proof relies on the simple observation that if \(T[a]\) through \(T[b]\) are all occupied and the run \emph{starts} in \(T[a]\) (i.e. \(T[a-1]\) is free which excludes the possibility of prior positions spilling over), then the preimage \(h^{-1}([a,b]) = \set{s \in S \, | \, h(x) \in [a, b]}\) must have size at least \(\size{b-a}\).
It must also be the case that either (1) the preimage \(h^{-1}([a+1, b])\) has size at least \((b-a)\cdot (1-\gamma) \) or (2) the preimage \(h^{-1}([a,a])\) is of size at least \((b-a)\cdot \gamma\), for any parameter \(\gamma \geq 0\).

We can generalize this to consider a run starting in any position \(T[b]\) within some interval \(b \in [a, c]\) which continues through \(T[d]\), then either (1) \(\size{h^{-1}([c, d])} \geq (d-c)\cdot(1-\gamma)\) or (2) \(\size{h^{-1}([a,c])} \geq (d-c) \cdot \gamma\).
We will refer to \([a,c]\) as the start-interval and to \([c, d]\) as the long interval.

Our strategy is to make both of these events unlikely by balancing the size of the start-interval with the number of keys needed to fill up the long interval.
Larger difference \((d-c)\) allows for a larger start-interval.
With a collection of roughly \(\log_{1+\eps/(6\alpha)} m\) such start-intervals we cover all possible starting poisitions before \(T[h(x) - \Delta]\), ruling out the possibility that a run starting before \(T[h(x)-\Delta]\) reaches \(T[h(x)]\).
The same strategy applied once more rules out the possibility that the run intersecting \(T[h(x)]\) will continue through \(T[h(x)+\Delta]\).

For our proof we set \(\gamma = \eps/3\) where \(\eps = 1 - n/m\) is the fill gap of \(T\).
The first pair of intervals we consider is the long interval \(I_0 = [h(x)-\Delta, h(x)]\) and the start-interval \(I_0'\) of size \(\Delta \eps/(6\alpha)\) preceding \(I_0\).
Next follows the long interval \(I_1 = I_0' \cup I_0\) with start-interval \(I_1'\) of length \(\size{I_1} \eps/(6\alpha)\) preceding it, and so forth.
Let \(\Delta_i = \size{I_i}\) and \(\Delta_i' = \size{I_i'}\). Observe how \(\Delta_i = \Delta \cdot (1 + \eps/(6\alpha))^i\), bounding the number of needed interval-pairs at \(\log_{1+\eps/(6\alpha)} (m/\Delta)\).

Depending on the length of the interval being inspected we can apply either \cref{lemma:upper-chernoff} or \cref{lemma:large-upper-chernoff} to bound the probability that the preimage exceeds the given threshold.
Taking the maximum of the two bounds simplifies the analysis.
Letting \(X\) be the size of a preimage, \(\mu = \Ep{X}\) and \(\delta \leq 1\) we obtain
\[
\Prp{X \geq (1+\delta) \mu} \leq \DepProb(\ssigma/2, d, \Sigma) + 4 \cdot \exp\ld(- \delta^2 \cdot \min\set{\ssigma/2, \mu}/3 \rd) \, .
\]

Let \(X_i\) be the size of the preimage of the long interval \(I_i\) of length \(\Delta_i\) with \(\mu_i = \alpha \Delta_i\).
Then
\begin{align*}
  \Prp{X_i \geq (1-\eps/3) \Delta_i} &= \Prp{X_i \geq \ld(1 + \frac{2 \eps}{3 \alpha}\rd) \alpha \Delta_i} \\
  &\leq \Prp{X_i \geq \ld(1 + \frac{2 \eps}{3}\rd) \mu_i} \\
  &\leq \DepProb(\ssigma/2, d, \Sigma) + 4 \cdot \exp\ld(- \ld(\frac{2\eps}{3}\rd)^2 \cdot \frac{\min\set{\mu_i, \ssigma/2}}{3} \rd)
\end{align*}
Notice how the probability is non-increasing for increasing sizes of the intervals. Thus we bound each of the probabilites for a long interval exceeding its threshold by the probability obtained for \(I_0\) with \(\mu_0 = \alpha \Delta \leq \ssigma/2\).

For start-interval \(I_i'\) of length \(\Delta_i'\) with \(\mu_i' = \alpha \Delta_i' = \Delta_i \cdot \eps/6\) we observe the same pattern
\begin{align*}
  \Prp{X_i' \geq \eps/3 \Delta_i} &= \Prp{X_i' \geq 2\mu_i'} \\
  &\leq \DepProb(\ssigma/2, d, \Sigma) + 4 \cdot \exp\ld(- \frac{\max\set{\mu_i', \ssigma/2}}{3}\rd) \, ,
\end{align*}
where we can bound the probability that each start-interval is too large by the probability obtained for \(I_0'\) with \(\mu_0' = \Delta \eps/6\).

The probability that \emph{any} of our intervals is too large is thus at most
\begin{align*}
  2 \log_{1 + \eps/(6\alpha)} m \cdot \ld( \DepProb(\ssigma/2, d, \Sigma) + 4 \exp\ld(- 4/27 \cdot \eps^2 \alpha \Delta\rd)\rd)
\end{align*}
where use that \(4/9 \cdot \eps^2 \alpha \Delta \leq \eps \Delta / 9 \leq \eps \Delta/6\) as \(\eps+\alpha=1\), hence the probability obtained for \(I_0\) is larger than that for \(I_0'\).

Let us rewrite this expression in terms of \(n\) and \(\ssigma\), our main parameters.
\begin{align*}
  \log_{1 + \eps/(6\alpha)} m &= \log_{1 + \eps/(6\alpha)} n + \log_{1 + \eps/(6\alpha)} (1/\alpha) \\
  &\leq \log n \cdot \log_{1 + \eps/(6\alpha)} (2) + 6 \\
  &\leq \log n \cdot 6 \alpha/\eps + 6 \\
  &\leq 30 \cdot \log n \, ,
\end{align*}
using \(\eps \geq 1/5\).
As \(\alpha \Delta \geq \ssigma/12\), we get
\begin{align*}
  4 \exp\ld(- 4/27 \cdot \eps^2 \alpha \Delta\rd) &\leq 4 \exp\ld(- 4/27 \cdot \eps^2 \ssigma/12\rd) \\
  &\leq 4 \exp\ld(- 1/2025 \cdot \ssigma\rd) \\
  &\leq \frac{1}{2\ssigma^2} \,
\end{align*}
as \(\ssigma \geq 2^{16}\).
Assuming \(30 \cdot \log n \leq \ssigma\) the total error-probability becomes
\[  1/(2\ssigma) + 30 \cdot \log n \cdot \DepProb(\ssigma/2, d, \Sigma) \, .\]

Repeating the process once more to ensure that the run at \(T[h(x)]\) doesn't continue past \(T[h(x) + \Delta]\) doubles the error-probability and proves the lemma.

\subsection{Proof of~\cref{cor:linearprobing}} \label{subsec:linearprobing-expectation}
To bound the expected number of comparisons we rely on the following lemma from \cite{patrascu12charhash} which gives strong concentration bounds for the runlength when applied to our simple tabulation \(\widehat h\).
\begin{lemma}[Corollary 3.2 in~\cite{patrascu12charhash}]\label{lemma:runlength}
 For any
  $\gamma=O(1)$ and $\ell\leq n^{1/(3(c+d))}/\alpha$,
\begin{align*}
\Pr[R(x,S)\geq \ell]\leq \left\{\begin{array}{ll}
2e^{-\Omega(\ell\eps^2)} + (\ell/m)^{\gamma} &\mbox{if }\alpha\geq 1/2\\
\alpha^{\Omega(\ell)} + (\ell/m)^{\gamma} &\mbox{if }\alpha\leq 1/2
\end{array}\right.
\end{align*}
where the constants hidden in \(O\) and \(\Omega\) are functions of \(c+d\), the size of the derived keys on which we apply simple tabulation.
\end{lemma}

In particular this implies that, for some $\ell = \Theta\ld((\log n)/\eps^2\rd)$, we have that $R(q,S)\geq \ell$ with probability at most $1/n^{10}$.
Let \(\calE\) be the event of stochastic dominance, as given by \cref{thm:linearprobing}, and \(\calA\) the event \((R(x, S) \leq \ell)\).
Then
\begin{align*}
  \Ep{X} &= \Epcond{X}{\calE} \cdot \Prp{\calE} + \Epcond{X}{\bar \calE \land \calA} \cdot \Prp{\bar \calE \land \calA} + \Epcond{X}{\bar \calE \land \bar \calA} \cdot \Prp{\bar \calE \land \bar \calA} \, .
\end{align*}
First, observe
\begin{align*}
  \Epcond{X}{\calE} \cdot \Prp{\calE} &= \sum_{i=1} \Prpcond{X \geq i}{\calE} \cdot \Prp{\calE} \\
  &\leq \sum_{i=1} \Prpcond{X^* \geq i}{\calE} \cdot \Prp{\calE} \\
  &= \sum_{i=1} \Prp{X^* \geq i \land \calE} \\
  &\leq \sum_{i=1} \Prp{X^* \geq i} \\
  &= \Ep{X^*} \, .
\end{align*}

With \(\delta = 1/\ssigma\) and \(d \geq 5\), \(\Prp{\bar \calE} \leq 9/\ssigma\).
Assuming \(\calA\), the next open cell of \(T\) is at most \(\ell\) positions away,
\begin{align*}
  \Epcond{X}{\bar \calE \land \calA} \cdot \Prp{\bar \calE \land \calA} &\leq \ell \cdot \Prp{\bar \calE} \\
  &\leq \Theta\ld(\frac{\log n}{\eps^2}\rd) \cdot \frac{9}{\ssigma} \\
  &\leq o(1) \, .
\end{align*}
Finally, no more than \(n\) comparisons will ever be necessary.
Hence
\begin{align*}
  \Epcond{X}{\bar \calE \land \bar \calA} \cdot \Prp{\bar \calE \land \bar \calA}
  &\leq n \cdot \Prp{\bar \calA} \\
  &\leq 1/n^{9} \, .
\end{align*}
This gives the desired bound on \(\Ep{X}\),
\begin{align*}
  \Ep{X} &\leq \Ep{X^*} + o(1) + 1/n^{9} \, .
\end{align*}

